Logit Attenuating Weight Normalization

Over-parameterized deep networks trained using gradient-based optimizers are a popular choice for solving classification and ranking problems. Without appropriately tuned $\ell_2$ regularization or weight decay, such networks have the tendency to make output scores (logits) and network weights large, causing training loss to become too small and the network to lose its adaptivity (ability to move around) in the parameter space. Although regularization is typically understood from an overfitting perspective, we highlight its role in making the network more adaptive and enabling it to escape more easily from weights that generalize poorly. To provide such a capability, we propose a method called Logit Attenuating Weight Normalization (LAWN), that can be stacked onto any gradient-based optimizer. LAWN controls the logits by constraining the weight norms of layers in the final homogeneous sub-network. Empirically, we show that the resulting LAWN variant of the optimizer makes a deep network more adaptive to finding minimas with superior generalization performance on large-scale image classification and recommender systems. While LAWN is particularly impressive in improving Adam, it greatly improves all optimizers when used with large batch sizes

==> sections/NotesForIntro.tex <==
\section{Introduction}
\label{sec:intro}

The deep learning community has witnessed an explosion of interest in training large deep neural networks (DNN) using large amounts of data. Examples include convolutional neural networks (CNNs) trained on millions of images (TODO cite ResNet, InceptionV3, AlexNet) and transformer (TODO cite transformer model) models trained on large text corpora (TODO cite BERT, ROBERTA, ALBERT). 

Typically, DNNs are trained using a optimizers like Adam (TODO Adam citation) and Stochastic Gradient Descent (SGD) (TODO add SGD citation)

We consider a class of neural networks known as \textit{homogeneous} neural networks. A homogeneous network $\mathbf{\phi}$ has the following property:
\begin{equation}
   \forall{\rho > 0}\quad  \phi(\rho x; \theta) = \rho \phi(\rho x; \theta)
\end{equation}
Many modern neural networks with ReLU (TODO citation) or Leaky ReLU (TODO citation) fall in this category. Examples include convolutional neural networks and feed forward neural networks. Although strict homogeneity excluded bias terms, there is evidence that inclusion of bias terms doesn't affect results in practice (TODO cite evidence). 


Our work is applicable only to homogeneous networks - layered networks with the property that multiplying all the weights of some l-th layer by a con- stant ρl will cause the final output of the network also to be multiplied by ρl. Thus, if we apply such a ρl factor to each layer, then the final output will get multiplied by Πlρl. Nets with ReLU or Leaky ReLU activation units belong to this class. Bias weights are disallowed from a strict homogeneous point of view, but, given that the number of such weights are small, it is fine to include them in practical implementations. In terms of weight groupings, we can include the bias weights associated with layer l with the weights in layer l.

\subsection{Motivation for layerwise normalization}


\subsection{Story 1}
We say that lawn is a general purpose extention to any kind of optimizer.
\begin{itemize}
    \item theory behind why it works?
    \item compare sgd (+lawn), adam (+lawn), lamb (+lawn) across multiple datasets.
    \item we might need to use logit norm to make sgd work and go into the details of scaling automatically.
\end{itemize}


\subsection{Story 2}
We restrict lawn to adam and pivot the story as follows:
\begin{itemize}
    \item Lawn makes adam work on any kind of data (nlp + recommender + images)
    \item Lawn makes adam work on any size of data, mini batch to full batch ~ not needing  lamb anymore
    \item showing that scaling weight norms helps but is not enough to make adam on its own work.
    \item explain why adam with lawn works with image dataset and it didnt before
\end{itemize}


Talk about 

\begin{itemize}
    \item Radial and lateral component
    \item Effect of network weights on margin
    \item Effect of batch size
\end{itemize}

We now motivate layer weight normalization. Consider a setup where a homogeneous neural network with an exponential loss function like cross entropy is being using an SGD-like algorithm. We also assume that the network is not using weight regularization (example: L2 regularization). Each mini-batch SGD gradient update has 2 components (1) a radial component that tries to increase the L2-norm of the weights and (2) a lateral component that increases the normalized margin. 

For a task like classification, for which a loss like cross entropy is well-suited, the radial component has very little role to . Moreover, as the networks weights grow 
Gradient updates for a method like SGD at every step have a radial component that tries to increase the norm of the weights and a lateral component that increases the margin. From the classifier performance point of view, the radial component plays little role since the direction associated with the weight vector is what really matters. Here is one way to see this. Let’s say that we have found one W that correctly classifies all training examples, i.e., $Margin > 0$. Now, if we take ρW , with ρ increasing from 1 towards ∞, then we can make the training loss go towards the perfect value of zero. This looks good from the training optimization point of view, but it is useless from the generalization performance point of view because the normalized margin doesn’t change at all, and so, if the original W had a poor
margin we don’t gain anything by moving purely radially.

We argue that 

the adaptive learning rate has undesirably large variance in
the early stage of model training,

Using story 2 for now



Why does Adam not work?

The adaptive learning rates used by Adam have a large variance during the early portion of model training (TODO cite Radam paper). Without weight regularizaton, the network weights grow rapidly. For homogeneous networks with exponential loss functions, the sample output probability $p_i$ depends on the magnitude of the parameter weights. The higher the weights, the more squised

==> sections/qualitative_analysis.tex <==
\section{Qualitative Analysis}
\label{sec:qualitative}

Some questions we want answered in this section:
\begin{itemize}
    \item How does the margin change during training? i.e. during the 3 phases (a) network separates the easy examples, (b) network gets 100\% training accuracy, (c) generalization \& improves test performance. we can use the alpha scaling on regular adam to show this.
    \item The escape phenomenon. i.e. there exists two parameters in the weight space that have same training loss but very different test performance. Therefore one of them have is more uniform and smooth. what experiment do we want to use to support this hypothesis?
    \item Are the minimas connected or isolated? i.e. once we reach the minima is it a question of traversing that path
    \item Lawn finds wider minima - does the hessian analysis show this?
    \item Isolatedness can be used to explain full batch success. we can show adam, starting from a point where adam-lawn has already reached inside the basin of attraction to show
    \item Toy Experiments: https://docs.google.com/document/d/10H3-C3N1QnhGArhHEnnr1Lo4vqf5wj2VflSM1kuYkZA/edit
\end{itemize}






